Parapuzzle of the Multibrot set and typical dynamics of unimodal maps

We study the parameter space of unicritical polynomials $f_c:z\mapsto z^d+c$. For complex parameters, we prove that for Lebesgue almost every $c$, the map $f_c$ is either hyperbolic or infinitely renormalizable. For real parameters, we prove that for Lebesgue almost every $c$, the map $f_c$ is either hyperbolic, or Collet-Eckmann, or infinitely renormalizable. These results are based on controlling the spacing between consecutive elements in the ``principal nest'' of parapuzzle pieces.

==> favprinc.tex <==
\begin{lemma}

If $V^{i_j-1} \subset Q^n$ and
$V^{i_j+1}$
is defined then $Q^{n+1}$ is defined and $V^{i_j+1} \subset
Q^{n+1}$.

\end{lemma}

\begin{pf}

Notice that $q_{n+1}=q_n+m'$
where $m$ is minimal with $f^m(0) \in P^n$ and
$\{f^k(0) :\ 1 \leq k \leq m\} \cap Q^n \setminus P^n \neq \emptyset$.
It is enough to show that $m \leq v_{i_j+1}-v_{i_j}$.
Notice that $V^{i_j} \subset P^n$, so
we just have to show that $\{f^k(0) :\ 1 \leq k \leq
v_{i_j+1}-v_{i_j}\} \cap Q^n \setminus P^n \neq \emptyset$.

%We have $\{f^k(0) :\ 1 \leq k \leq v_{i_j+1}-v_{i_j}\} \cap V^{i_j-1}
%\setminus V^{i_j} \neq \emptyset$.

Let $k \geq 1$ be minimal such that $f^k(0) \in Q^n \setminus P^n$.
Then $k=l_0(p_n-q_n)$ for some $l_0>0$, and
$R_{Q^n}^l(0) \in Y^{q_n+(l_0-l)(p_n-q_n)} \setminus
Y^{p_n+(l_0-l)(p_n-q_n)}$, $1 \leq l \leq l_0$.

Notice that $R_{Q^n}(0) \notin V^{i_j}$, so that $V^{i_j} \subset
Y^{q_n+(l_0-1)(p_n-q_n)}$.  This clearly implies that
$R_{Q^n}^l(0) \notin V^{i_j}$, $1 \leq l \leq l_0$, so $v_{i_j+1}-v_{i_j}
\geq k$, as desired.
\end{pf}


